Autonomous Racing with AutoRally Vehicles and Differential Games

Safe autonomous vehicles must be able to predict and react to the drivers around them. Previous control methods rely heavily on pre-computation and are unable to react to dynamic events as they unfold in real-time. In this paper, we extend Model Predictive Path Integral Control (MPPI) using differential game theory and introduce Best-Response MPPI (BR-MPPI) for real-time multi-vehicle interactions. Experimental results are presented using two AutoRally platforms in a racing format with BR-MPPI competing against a skilled human driver at the Georgia Tech Autonomous Racing Facility.

==> commands.tex <==
%% definitions used in proposal

\newtheoremstyle{break}
  {\topsep}{\topsep}%
  {\itshape}{}%
  {\bfseries}{}%
  {\newline}{}%

\theoremstyle{break}
%\newtheorem{theorem}{Theorem}

%%%%%%%%5
\DeclareMathOperator*{\E}{\mathbb{E}}
\DeclareMathOperator{\Tr}{tr}


\newcommand{\dx}{\mathrm{d}x}
\newcommand{\dt}{\mathrm{d}t}
\newcommand{\dw}{\mathrm{d}w}
\newcommand{\dtau}{\mathrm{d}\tau}
\newcommand{\dq}{\mathrm{d}q}

\newcommand{\dV}{\mathrm{d}V}
\newcommand{\dif}[1]{\mathrm{d}{#1}}
%%%%%%%%
%%: Variable Names
\newcommand{\prob}{\mathbb{P}}  % Reals
\newcommand{\reals}{\mathbb{R}}  % Reals
\newcommand{\PrcOnObstacle}{\mathtt{OnObstacle}}
\newcommand{\Xappfree}{\widehat{\X}_{\mathrm{free}}} %Free Configuration space
\newcommand{\Xappobs}{\widehat{\X}_{\mathrm{obs}}} %Free Configuration space

\newcommand{\True}{{\tt True}}
\newcommand{\False}{{\tt False}}
\newcommand{\PrcDensityEstimator}{\mathtt{DensityEstimator}}
\newcommand{\PrcClassifier}{\mathtt{Classifier}}

\newcommand{\fBeliefObsPdf}{b_{\mathrm{obs}}}
\newcommand{\fBeliefFreePdf}{b_{\mathrm{free}}}
\newcommand{\qFree}{q_{\mathrm{free}}}
\newcommand{\qObs}{q_{\mathrm{obs}}}

\newcommand{\priorFree}{\pi_{\mathrm{free}}}
\newcommand{\priorObs}{\pi_{\mathrm{obs}}}
\newcommand{\XFreeList}{X_{\mathrm{free}}} 
\newcommand{\XObsList}{X_{\mathrm{obs}}} 
\newcommand{\XSampleList}{X_{\mathrm{sample}}} 
\newcommand{\X}{\mathcal{X}} 		%Configuration space
\newcommand{\classLabel}{\mathtt{label}}
%%%%%%%

%%: ALGORITHM NAMES

\newcommand{\AlgRRT}{\ensuremath{{\mathrm{RRT}}}}
\newcommand{\AlgPRM}{\ensuremath{{\mathrm{PRM}}}}
\newcommand{\AlgRRG}{\ensuremath{{\mathrm{RRG}}}}
\newcommand{\AlgPRMstar}{\ensuremath{{\mathrm{PRM}^*}}}
\newcommand{\AlgRRTstar}{\ensuremath{{\mathrm{RRT}^*}}}
\newcommand{\AlgRRTsharp}{\ensuremath{{\mathrm{RRT}^\#}}}
\newcommand{\AlgRRTrtdp}{\ensuremath{{\mathrm{RRT}^{\mathrm{rt}}}}}
\newcommand{\AlgRRTsharpNoBlackVertex}{\ensuremath{{\mathrm{RRT}^\#_{1}}}}
\newcommand{\AlgRRTsharpPromisingParent}{\ensuremath{{\mathrm{RRT}^\#_{2}}}}
\newcommand{\AlgRRTsharpPromisingNewVertex}{\ensuremath{{\mathrm{RRT}^\#_{3}}}}
\newcommand{\AlgExtendRRTsharp}{\ensuremath{{\tt Extend}_{RRT^\#}}}





%% New Definitions
\definecolor{gray}{RGB}{190,190,190}
\definecolor{darkgreen}{rgb}{0,0.5,0} \newcommand{\dg}{\color{darkgreen}}
\definecolor{fullred}{rgb}{0.85,.0,.1} \newcommand{\fr}{\color{fullred}}
\definecolor{brown}{rgb}{0.65,0.16,0.16} \newcommand{\br}{\color{brown}}
\definecolor{mybrown}{RGB}{255,218,195}
\definecolor{myframe}{RGB}{197,122,195}

% New Commands


%%%% newly included

\newcommand{\graphGrid}{\graph{G}_{\mathrm{grid}}}
\newcommand{\vertexGrid}{\vertex{V}_{\mathrm{grid}}}
\newcommand{\edgeGrid}{\edge{E}_{\mathrm{grid}}}

\newcommand{\U}{\mathcal{U}} 		%Controls space
\newcommand{\ti}{t_{\mathrm{i}}} 	% initial time
\newcommand{\tf}{t_{\mathrm{f}}}	% final time
\newcommand{\xin}{x_{\mathrm{i}}}	% initial state
\newcommand{\xfn}{x_{\mathrm{f}}}	% final state

\newcommand{\Xapp}{\widehat{\mathcal{X}}} 		%Configuration space

\newcommand{\PrcKeyApp}{\widehat{\mathtt{Key}}} % Parent procedure for a vertex x on a graph
\newcommand{\Xgrid}{\X_{\mathrm{grid}}} %Free Configuration space
\newcommand{\Xapprel}{\widehat{\X}_{\mathrm{rel}}} %Free Configuration space
\newcommand{\Xappgoal}{\widehat{\X}_{\mathrm{goal}}} %Free Configuration space
\newcommand{\gAppValue}{\widehat{\mathtt{g}}}			% g-value of the state x	
\newcommand{\gAppStarValue}{\widehat{\mathtt{g}}^{*}}	% g* value of the state x
\newcommand{\xappmingoal}{\widehat{x}^{*}_{\mathrm{goal}}}	% goal point in Xgoal with minimum g*-value	



\newcommand{\Neigh}{\mathcal{N}}
\newcommand{\Neighapp}{\widehat{\mathcal{N}}}






%%%%
%%: Variable Names
\newcommand{\integers}{\mathbb{Z}} % Integers (Z is positive/negative integers, and 0, right?)
\newcommand{\naturals}{\mathbb{N}} 	% Natural numbers
\newcommand{\Xfree}{\X_{\mathrm{free}}} %Free Configuration space
\newcommand{\Xgoal}{\X_{\mathrm{goal}}} % Goal set in the configuration space
\newcommand{\Xobs}{\X_{\mathrm{obs}}} 	% Obstacle region in the configuration space
\newcommand{\Xrel}{\X_{\mathrm{rel}}} 	% Relevant configuration space

\newcommand{\Xbox}{\X_{\mathrm{box}}} 	% Relevant configuration space

\newcommand{\xrand}{x_{\mathrm{rand}}}	% randomly sampled state x
\newcommand{\xnew}{x_{\mathrm{new}}}	% new state x	
\newcommand{\xinit}{x_{\mathrm{init}}}	% initial state x	
\newcommand{\xgoal}{x_{\mathrm{goal}}}	% goal state x	
\newcommand{\xnearest}{x_{\mathrm{nearest}}}	% initial state x
\newcommand{\xmingoal}{x^{*}_{\mathrm{goal}}}	% goal point in Xgoal with minimum g*-value	

\newcommand{\tree}[1]{\mathcal{#1}} 		% Tree data structure
\newcommand{\graph}[1]{\mathcal{#1}}		% Graph data structure
\newcommand{\vertex}[1]{\mathcal{#1}}		% vertex set
\newcommand{\edge}[1]{\mathcal{#1}}		% edge set


\newcommand{\vgoal}{v_{\mathrm{goal}}}	% Goal vertex set
\newcommand{\Vgoal}{V_{\mathrm{goal}}}	% Goal vertex set

\newcommand{\Iall}{I}					% Indices of goal vertices
\newcommand{\Igoal}{I_{\mathrm{goal}}}	% Indices of goal vertices

\newcommand{\Vprom}{V_{\mathrm{prom}}}	% Promising vertices
\newcommand{\Vexp}{V_{\mathrm{exp}}}	% Promising vertices
\newcommand{\vmingoal}{v^{*}_{\mathrm{goal}}}	% goal vertex in Xgoal with minimum key value	
\newcommand{\vappmingoal}{\widehat{v}^{*}_{\mathrm{goal}}}	% goal vertex in Xgoal with minimum key value	
\newcommand{\vprimegoal}{v^{*}_{\mathrm{goal}}}	% goal vertex in Xgoal with minimum key value	
%\newcommand{\vprimegoal}{v^{\prime}_{\mathrm{goal}}}	% goal vertex in Xgoal with minimum key value	



\newcommand{\VValue}{\mathtt{V}}						% locally minimum cost-to-come of state x
\newcommand{\VctgValue}{\mathtt{V}_{\mathrm{ctg}}}		% locally minimum cost-to-come of state x
\newcommand{\VctcValue}{\mathtt{V}_{\mathrm{ctc}}}		% locally minimum cost-to-come of state x
\newcommand{\VctgStarValue}{\mathtt{V}^{*}_{\mathrm{ctg}}}		% locally minimum cost-to-come of state x
\newcommand{\VctcStarValue}{\mathtt{V}^{*}_{\mathrm{ctc}}}		% locally minimum cost-to-come of state x
\newcommand{\JValue}{\mathtt{J}}						% locally minimum cost-to-come of state x
\newcommand{\JStarValue}{\mathtt{J^{*}}}				% locally minimum cost-to-come of state x

\newcommand{\lmcValue}{\mathtt{lmc}}					% locally minimum cost-to-come of state x
\newcommand{\lmcAppValue}{\widehat{\mathtt{lmc}}}	% g* value of the state x
\newcommand{\fValue}{\mathtt{f}}						% f-value of the state x
\newcommand{\fPrimeValue}{\mathtt{f}}			% f-value of the state x
%\newcommand{\fPrimeValue}{\mathtt{f^{\prime}}}			% f-value of the state x




\newcommand{\gValue}{\mathtt{g}}			% g-value of the state x	
%\newcommand{\gPrimeValue}{\mathtt{g^{\prime}}}	% g-dag value of the state x
\newcommand{\gPrimeValue}{\mathtt{g^{*}}}	% g-dag value of the state x	
\newcommand{\gStarValue}{\mathtt{g^{*}}}	% g* value of the state x
\newcommand{\hValue}{\mathtt{h}}			% heuristic-value of the state x
\newcommand{\costValue}{\mathtt{c}}			% cost-value of the path

\newcommand{\PrcSample}{\mathtt{Sample}} % Sample procedure
\newcommand{\PrcExtend}{\mathtt{Extend}} % Extend procedure
\newcommand{\PrcNearest}{\mathtt{Nearest}} % Nearest procedure
\newcommand{\PrcNear}{\mathtt{Near}}      % Near procedure
\newcommand{\PrcSteer}{\mathtt{Steer}}   % Steer procedure
\newcommand{\PrcLine}{\mathtt{Line}}   % Line procedure
\newcommand{\PrcObstacleFree}{\mathtt{ObstacleFree}} %ObstacleFree procedure
\newcommand{\PrcReplan}{\mathtt{Replan}} %ReduceInconsistency procedure
%\newcommand{\PrcReduceInconsistency}{\mathtt{ReduceInconsistency}} %ReduceInconsistency procedure
\newcommand{\PrcReduceInconsistency}{\mathtt{Replan}} %ReduceInconsistency procedure
\newcommand{\PrcUpdateState}{\mathtt{UpdateQueue}} %UpdateState procedure
\newcommand{\PrcIncludeVertex}{\mathtt{IncludeVertex}} %UpdateState procedure

\newcommand{\PrcSuccessor}{\mathtt{succ}} % Successor procedure for a vertex x on a graph
\newcommand{\PrcPredecessor}{\mathtt{pred}} % Predecessor procedure for a vertex x on a graph
\newcommand{\PrcParent}{\mathtt{parent}} % Parent procedure for a vertex x on a graph
\newcommand{\PrcKey}{\mathtt{Key}} % Parent procedure for a vertex x on a graph




%%: Useful Commands
\newcommand{\hideMaterial}[1]{}
\newcommand{\hideoldproofofnegresult}[1]{ }

%\newcommand{\note}[2]{
%{\color{gray}``#2''},$^{{\color{red}\mathrm{#1}}}$
%}

%\newcommand{\todo}[1]{
%{\color{red}``#1''}
%}

\newcommand{\myalert}[1]{
{\color{red} #1}
}



==> mppi_math.tex <==
\newcommand{\rd}{{\mathrm d}}
\newcommand{\rdelta}{{\mathrm \delta}}
\newcommand{\rtr}{{\mathrm{tr}}}
\newcommand{\rP}{{\mathrm{P}}}
\newcommand{\rT}{{\mathrm{T}}}
\newcommand{\rvec}{{\mathrm{vec}}}
\newcommand{\rtau}{{\mathrm{\tau}}}
\newcommand{\vx}{{\bf x}}
\newcommand{\vy}{{\bf y}}
\newcommand{\vk}{{\bf k}}
\newcommand{\vG}{{\bf G}}
\newcommand{\vu}{{\bf u}}
\newcommand{\va}{{\bf a}}
\newcommand{\vw}{{\bf w}}
\newcommand{\vf}{{\bf f}}
\newcommand{\vA}{{\bf A}}
\newcommand{\vR}{{\bf R}}
\newcommand{\vE}{{\bf E}}
\newcommand{\vF}{{\bf F}}
\newcommand{\vL}{{\bf L}}
\newcommand{\vI}{{\bf I}}
\newcommand{\vK}{{\bf K}}
\newcommand{\vJ}{{\bf J}}
\newcommand{\vM}{{\bf M}}
\newcommand{\vD}{{\bf D}}
\newcommand{\vN}{{\bf N}}
\newcommand{\vV}{{\bf V}}
\newcommand{\vH}{{\bf H}}
\newcommand{\vT}{{\bf T}}
\newcommand{\vC}{{\bf C}}
\newcommand{\vO}{{\bf O}}
\newcommand{\vQ}{{\bf Q}}
\newcommand{\vB}{{\bf B}}
\newcommand{\vS}{{\bf S}}
\newcommand{\vX}{{\bf X}}
\newcommand{\vY}{{\bf Y}}
\newcommand{\vP}{{\bf P}}
\newcommand{\rank}{{\text{rank}}}
\newcommand{\vect}{{\text{vec}}}
\newcommand{\vxi}{{\mbox{\boldmath$\xi$}}}
\newcommand{\vpi}{{\mbox{\boldmath$\pi$}}}
\newcommand{\vdomega}{{\bf d\omega}}
\newcommand{\vlambda}{{\mbox{\boldmath$\lambda$}}}
\newcommand{\vBamma}{{\mbox{\boldmath$\Gamma$}}}
\newcommand{\VTheta}{{\mbox{\boldmath$\Theta$}}}
\newcommand{\VPhi}{{\mbox{\boldmath$\Phi$}}}
\newcommand{\vphi}{{\mbox{\boldmath$\phi$}}}
\newcommand{\VPsi}{{\mbox{\boldmath$\Psi$}}}
\newcommand{\ve}{{\mbox{\boldmath$\epsilon$}}}
\newcommand{\VSigma}{{\mbox{\boldmath$\Sigma$}}}
\newcommand{\valpha}{{\mbox{\boldmath$\alpha$}}}
\newcommand{\vmu}{{\mbox{\boldmath$\mu$}}}
\newcommand{\vbeta}{{\mbox{\boldmath$\beta$}}}
\newcommand{\vomega}{{\mbox{\boldmath$\omega$}}}
\newcommand{\vtau}{{\mbox{\boldmath$\tau$}}}
\newcommand{\vdtau}{{\mbox{\boldmath$d\tau$}}}
\newcommand{\vtheta}{{\mbox{\boldmath$\theta$}}}\newcommand{\dataset}{{\cal D}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\vcalS}{{\mbox{\boldmath$\cal{S}$}}}
\newcommand{\vcalU}{{\mbox{\boldmath$\cal{U}$}}}
\newcommand{\vcalD}{{\mbox{\boldmath$\cal{D}$}}}
\newcommand{\vcalJ}{{\mbox{\boldmath$\cal{J}$}}}
\newcommand{\vcalE}{{\mbox{\boldmath$\cal{E}$}}}
\newcommand{\vcalF}{{\mbox{\boldmath$\cal{F}$}}}
\newcommand{\vcalL}{{\mbox{\boldmath$\cal{L}$}}}
\newcommand{\vcalZ}{{\mbox{\boldmath$\cal{Z}$}}}
\newcommand{\vcalG}{{\mbox{\boldmath$\cal{G}$}}}
\newcommand{\vcalN}{{\mbox{\boldmath$\cal{N}$}}}
\newcommand{\vcalM}{{\mbox{\boldmath$\cal{M}$}}}
\newcommand{\vcalH}{{\mbox{\boldmath$\cal{H}$}}}
\newcommand{\vcalC}{{\mbox{\boldmath$\cal{C}$}}}
\newcommand{\vcalO}{{\mbox{\boldmath$\cal{O}$}}}
\newcommand{\vcalP}{{\mbox{\boldmath$\cal{P}$}}}
\newcommand{\vcalB}{{\mbox{\boldmath$\cal{B}$}}}
\newcommand{\vcalA}{{\mbox{\boldmath$\cal{A}$}}}
\newcommand{\vcalg}{{\mbox{\boldmath$\cal{g}$}}}
\newcommand{\calN}{\mbox{$\cal{N}$}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\T}{^\mathsf{T}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calA}{\mathcal{A}}

\newcommand{\Qb}{\mathbb{Q}}
\newcommand{\Eb}{\mathbb{E}}
\newcommand{\Pb}{\mathbb{P}}
\newcommand{\Rb}{\mathbb{R}}
\newcommand{\Xspace}{\mathcal{X}}
\newcommand{\snew}{\mathbf{x}^\prime}
\newcommand{\s}{\mathbf{x}}
\newcommand{\Pas}[2]{\mathcal{P}\left({#1}|{#2}\right)}
\newcommand{\Pol}[2]{\mathcal{U}\left({#1}|{#2}\right)}
\newcommand{\PolOpt}[2]{\mathcal{U}^{*}\left({#1}|{#2}\right)}
\newcommand{\PolPasT}[1]{\mathcal{P}\left({#1}\right)}
\newcommand{\PolT}[1]{\mathcal{U}\left({#1}\right)}
\newcommand{\traj}{\mathbf{X}}
\newcommand{\KL}[2]{\mathbb{D}_{KL}\left({#1}\parallel {#2}\right)}
\newcommand{\costt}[1]{\mathcal{J}\left({#1}\right)}
\newcommand{\logb}[1]{\log\left({#1}\right)}
\newcommand{\expb}[1]{\exp\left({#1}\right)}
\newcommand{\val}[2]{\mathit{V}_{#2}\left({#1}\right)}
\newcommand{\zt}[2]{\Phi_{#2}\left({#1}\right)}
\newcommand{\nZ}[2]{\mathcal{G}_t[\Phi]\left({#1}\right)}
\newcommand{\ExP}[2]{\E_{{#1}}{\left[#2\right]}}
